Machine learning search for variable stars

Photometric variability detection is often considered as a hypothesis testing problem: an object is variable if the null-hypothesis that its brightness is constant can be ruled out given the measurements and their uncertainties. Uncorrected systematic errors limit the practical applicability of this approach to high-amplitude variability and well-behaving data sets. Searching for a new variability detection technique that would be applicable to a wide range of variability types while being robust to outliers and underestimated measurement uncertainties, we propose to consider variability detection as a classification problem that can be approached with machine learning. We compare several classification algorithms: Logistic Regression (LR), Support Vector Machines (SVM), k-Nearest Neighbors (kNN) Neural Nets (NN), Random Forests (RF) and Stochastic Gradient Boosting classifier (SGB) applied to 18 features (variability indices) quantifying scatter and/or correlation between points in a light curve. We use a subset of OGLE-II Large Magellanic Cloud (LMC) photometry (30265 light curves) that was searched for variability using traditional methods (168 known variable objects identified) as the training set and then apply the NN to a new test set of 31798 OGLE-II LMC light curves. Among 205 candidates selected in the test set, 178 are real variables, 13 low-amplitude variables are new discoveries. We find that the considered machine learning classifiers are more efficient (they find more variables and less false candidates) compared to traditional techniques that consider individual variability indices or their linear combination. The NN, SGB, SVM and RF show a higher efficiency compared to LR and kNN.

==> Makefile <==
all: clean mlvid.pdf

clean: 
	rm -f mlvid.bbl  mlvid.pdf mlvid.ps mlvid.dvi mlvid.log mlvid.aux mlvid.blg DEADJOE *~ *.bak main_paper.pdf online_material.pdf mlvid.out mlvid.teximulated mn2e.bst_backup

mlvid.pdf: mlvid.tex
	# This works with .eps figures or when \usepackage[demo]{graphicx} is activated
	latex mlvid.tex && latex mlvid.tex && bibtex mlvid && latex mlvid.tex && latex mlvid.tex && dvips -o mlvid.ps mlvid.dvi && ps2pdf mlvid.ps && okular mlvid.pdf
	# This works with .png figures
	#pdflatex mlvid.tex && pdflatex mlvid.tex && bibtex mlvid && pdflatex mlvid.tex && pdflatex mlvid.tex && okular mlvid.pdf
	
